Multiscale Gossip for Efficient Decentralized Averaging in Wireless Packet Networks

This paper describes and analyzes a hierarchical gossip algorithm for solving the distributed average consensus problem in wireless sensor networks. The network is recursively partitioned into subnetworks. Initially, nodes at the finest scale gossip to compute local averages. Then, using geographic routing to enable gossip between nodes that are not directly connected, these local averages are progressively fused up the hierarchy until the global average is computed. We show that the proposed hierarchical scheme with $k$ levels of hierarchy is competitive with state-of-the-art randomized gossip algorithms, in terms of message complexity, achieving $\epsilon$-accuracy with high probability after $O\big(n \log \log n \log \frac{kn}{\epsilon} \big)$ messages. Key to our analysis is the way in which the network is recursively partitioned. We find that the optimal scaling law is achieved when subnetworks at scale $j$ contain $O(n^{(2/3)^j})$ nodes; then the message complexity at any individual scale is $O(n \log \frac{kn}{\epsilon})$, and the total number of scales in the hierarchy grows slowly, as $\Theta(\log \log n)$. Another important consequence of hierarchical construction is that the longest distance over which messages are exchanged is $O(n^{1/3})$ hops (at the highest scale), and most messages (at lower scales) travel shorter distances. In networks that use link-level acknowledgements, this results in less congestion and resource usage by reducing message retransmissions. Simulations illustrate that the proposed scheme is more message-efficient than existing state-of-the-art randomized gossip algorithms based on averaging along paths.

==> model.tex <==
 Let $G = (V,E)$ be a random geometric graph \cite{penroseRGG} of $n$ nodes with connectivity radius $r_{con}(n)$. Each node in $G$ holds an initial real value $x_{i}(0)$. Vector $x(t) = [x_{1}(t) x_{2}(t) \dots x_{n}(t)]^{\mbox{T}}$ describes the values on the network at time $t$. Our goal is for nodes to communicate over graph edges to compute the average $x_{ave} = \frac{1}{n}\sum_{i=1}^{n} x_{i}(0)$. In the end, all nodes should have knowledge of $x_{ave}$. To measure performance of an averaging algorithm we use the following definition.

\begin{dfn}
$\epsilon$ \textit{averaging time} $T_{\epsilon}(n)$. Given any desired accuracy $\epsilon > 0$, the $\epsilon$ \textit{averaging time} is the earliest time at which vector $x(t)$ is $\epsilon$ close to the normalized true average with probability greater than $1-\epsilon$:
\end{dfn}

\begin{equation}
T_{\epsilon}(n) = \mbox{sup}_{x(0)} \mbox{inf}_{t=0,1,2, \ldots } \left\{ \mathbb{P} \left( \frac{|| x(t) - x_{ave} || }{||x(0)||} \geq \epsilon \right) \leq \epsilon \right\}
\end{equation}

Convergence rate generally depends on the initial values $x(0)$ and the definition assumes the worst possible starting point. In practice, to eliminate the possibility of favourable initial conditions  when evaluating our algorithm, as initial condition we assign to each node the sum of its geographic coordinates\footnote{Although not formally proven, we observed that this initial condition is harder than assigning zero velues to all nodes except one or uniform random assignment which are popular alternatives.}.

Notice that time is measured in discrete time moments until convergence. As explained in \cite{Boyd06} this facilitates the analysis of gossip algorithms but does not force the actual implementation to be sequential. Multiple communication events happen in parallel. Finally, for multi-scale gossip we use $T_{\epsilon}(n)$ since the consensus time characterization of convergence rate defined in \cite{denantes08} is not applicable. Specifically, our averaging scheme proceeds in phases and changes over time in a non-ergodic manner. Moreover, by definition our scheme stops after a finite number of iterations.  The approach in \cite{denantes08} is only defined asymptotically as $t \rightarrow \infty$  and for averaging schemes that are ergodic.


